Hierarchical Patch Diffusion Models for High-Resolution Video Generation

Diffusion models have demonstrated remarkable performance in image and video synthesis. However, scaling them to high-resolution inputs is challenging and requires restructuring the diffusion pipeline into multiple independent components, limiting scalability and complicating downstream applications. This makes it very efficient during training and unlocks end-to-end optimization on high-resolution videos. We improve PDMs in two principled ways. First, to enforce consistency between patches, we develop deep context fusion -- an architectural technique that propagates the context information from low-scale to high-scale patches in a hierarchical manner. Second, to accelerate training and inference, we propose adaptive computation, which allocates more network capacity and computation towards coarse image details. The resulting model sets a new state-of-the-art FVD score of 66.32 and Inception Score of 87.68 in class-conditional video generation on UCF-101 $256^2$, surpassing recent methods by more than 100%. Then, we show that it can be rapidly fine-tuned from a base $36\times 64$ low-resolution generator for high-resolution $64 \times 288 \times 512$ text-to-video synthesis. To the best of our knowledge, our model is the first diffusion-based architecture which is trained on such high resolutions entirely end-to-end. Project webpage: https://snap-research.github.io/hpdm.

==> figures/fvd-clipscore-curve.tex <==
\begin{figure}
\centering
\includegraphics[width=\linewidth,height=3cm]{example-image-a}
\label{fig:fvd-clipscore-curve}
\end{figure}


==> figures/inference.tex <==
\begin{figure*}
% \centering
% \begin{subfigure}[b]{0.33\textwidth}
%     \centering
%     \includegraphics[width=\textwidth, height=5cm]{example-image-a}
% \end{subfigure}
% \hfill
% \begin{subfigure}[b]{0.66\textwidth}
%     \centering
%     \includegraphics[width=\textwidth, height=5cm]{example-image-a}
% \end{subfigure}
\includegraphics[width=\linewidth]{images/inference.pdf}
\caption{Effect of the overlapped inference~\cite{MultiDiffusion} (left) and its effects on the consistency between the patches (right). Surprisingly, even without the full-resolution training~\cite{PatchDiffusion} and patch overlapping, our deep context fusion strategy manages to preserve strong consistency in the generated sample.}
\label{fig:inference}
\end{figure*}


==> figures/patch-extraction.tex <==
\begin{figure}
\centering
\includegraphics[width=0.6\linewidth]{images/patch-extraction.pdf}
\caption{Illustration of the patch extraction procedure for 2D case. We use the same pipeline as \cite{EpiGRAF} and extract the patches based on random scale $s$ and offsets $\delta_f,\delta_h,\delta_w$.}
\label{fig:patch-extraction}
\end{figure}

